HEALTH-PARIKSHA: Assessing RAG Models for Health Chatbots in Real-World Multilingual Settings

Assessing the capabilities and limitations of large language models (LLMs) has garnered significant interest, yet the evaluation of multiple models in real-world scenarios remains rare. Multilingual evaluation often relies on translated benchmarks, which typically do not capture linguistic and cultural nuances present in the source language. This study provides an extensive assessment of 24 LLMs on real world data collected from Indian patients interacting with a medical chatbot in Indian English and 4 other Indic languages. We employ a uniform Retrieval Augmented Generation framework to generate responses, which are evaluated using both automated techniques and human evaluators on four specific metrics relevant to our application. We find that models vary significantly in their performance and that instruction tuned Indic models do not always perform well on Indic language queries. Further, we empirically show that factual correctness is generally lower for responses to Indic queries compared to English queries. Finally, our qualitative work shows that code-mixed and culturally relevant queries in our dataset pose challenges to evaluated models.

==> sections/7_limitations.tex <==
\section{Limitations}
\label{sec:limitations}

Our work is subject to several limitations. 

\begin{itemize}
\item Because our dataset is derived from actual users of a healthcare bot, we couldn't regulate the ratio of English to non-English queries. Consequently, the volume of non-English queries in our dataset is significantly lower than that of English queries, meaning the results on non-English queries should not be considered definitive. Similarly, since the \textsc{HealthBot} is available only in four Indian languages, we also could not evaluate on languages beyond these. The scope of our \textsc{HealthBot} setting is currently confined to queries from patients at one hospital in India, resulting in less varied data. We intend to expand this study as \textsc{HealthBot} extends its reach to other parts of the country.
\item While we evaluated numerous models in this work, some were excluded from this study for various reasons, such as ease of access. We aim to incorporate more models in future research.
\item Research has indicated that LLM-based evaluators tend to prefer their own responses. In our evaluations, we use \textsc{GPT-4o}, and there may be a bias leading to higher scores for the \textsc{GPT-4o} model and other models within the GPT family. Although not investigated in prior research, it is also conceivable that models fine-tuned with synthetic data generated by \textsc{GPT-4o} might receive elevated scores. We urge readers to keep these in mind while interpreting the scores. In future work, we plan to use multiple LLM-evaluators to obtain more robust results.
\item Finally, our human evaluation was limited to a subset of models and data, and a single metric due to time and budget constraints. In future work, we plan to incorporate more human evaluation, as well as qualitative analysis of the results.
\end{itemize}
